Machine Learning Visualization Tool for Exploring Parameterized Hydrodynamics

We are interested in the computational study of shock hydrodynamics, i.e. problems involving compressible solids, liquids, and gases that undergo large deformation. These problems are dynamic and nonlinear and can exhibit complex instabilities. Due to advances in high performance computing it is possible to parameterize a hydrodynamic problem and perform a computational study yielding $\mathcal{O}\left({\rm TB}\right)$ of simulation state data. We present an interactive machine learning tool that can be used to compress, browse, and interpolate these large simulation datasets. This tool allows computational scientists and researchers to quickly visualize "what-if" situations, perform sensitivity analyses, and optimize complex hydrodynamic experiments.

==> makefile <==
DOC  := jekel_mlviz_rev00.tex

RERUN := "(undefined references|Rerun to get (cross-references|the bars|point totals) right|Table widths have changed. Rerun LaTeX.|Linenumber reference failed)"
RERUNBIB := "No file.*\.bbl|Citation.*undefined"

# all: figs doc
all: doc

figs:
	@$(MAKE) -C $@

doc: $(DOC:.tex=.pdf)

%.pdf: %.tex
	pdflatex $<
	@egrep -q $(RERUNBIB) $*.log && bibtex $* && pdflatex $<; true
	@egrep -q $(RERUN) $*.log && pdflatex $<; true
	@egrep -q $(RERUN) $*.log && pdflatex $<; true

latexmk:
	-latexmk -pvc -pdf $(DOC)

purge:
	-rm -f *.{aux,dvi,log,bbl,blg,brf,fls,toc,thm,out,fdb_latexmk}

clean: purge
	# $(MAKE) -C figs $@
	-rm -f $(DOC:.tex=.pdf)

.PHONY: all figs purge clean
